Pinpointing Delay and Forwarding Anomalies Using Large-Scale Traceroute Measurements

Understanding network health is essential to improve Internet reliability. For instance, detecting disruptions in peer and provider networks facilitates the identification of connectivity problems. Currently this task is time consuming for network operators. It involves a fair amount of manual observation because operators have little visibility into other networks. In this paper we leverage the RIPE Atlas measurement platform to monitor and analyze network conditions. We propose a set of complementary methods to detect network disruptions from traceroute measurements. A novel method of detecting changes in delays is used to identify congested links, and a packet forwarding model is employed to predict traffic paths and to identify faulty routers in case of packet loss. In addition, aggregating results from each method allows us to easily monitor a network and identify coordinated reports manifesting significant network disruptions, reducing uninteresting alarms. Our contributions consist of a statistical approach providing robust estimation for Internet delays and the study of hundreds of thousands link delays. We present three cases demonstrating that the proposed methods detect real disruptions and provide valuable insights, as well as surprising findings, on the location and impact of identified events.

==> discussions.tex <==

\section{Discussion}


%Mapping our results to infrastructure \cite{giotsas:conext15} would be great.
%ICMP traffic


==> related_works.tex <==

\section{Related Works}
\todo{related works}
Outage detection (control plane) \cite{trinocular}
Interdomain congestion \cite{luckie:imc14}
\begin{itemize}
    \item Only the inter-domain links near the probes
    \item Only when the return path go through the monitored link (29.9\%)
\end{itemize}

visualization tools \cite{kisteleki:amsix15, manojlovic:sanog16}

Reverse traceroute \cite{katz:nsdi10} \cite{marchetta:pam14}

RTT multimodal distribution \cite{romain:infocom15}

Locating Congestion:
use two ways RTT \cite{chand:conext15}

Delays estimations \cite{lee:infocom10}

ICMP option: tulip \cite{mahajan:sosp03}, cing \cite{cing:infocom03}

congestion detection through packet loss analysis \cite{sommers:sigcomm05}
modelling/study on packet loss \cite{yajnik:infocom99,gu:infocom09}

Forwarding anomalies
Cite \cite{dhamdhere:imc10}








Cite \cite{dhamdhere:imc10}
\cite{yajnik:infocom99}

cing \cite{cing:infocom03}

